Constraint Satisfaction Problems over Finitely Bounded Homogeneous Structures: a Dichotomy between FO and L-hard

Feder-Vardi conjecture, which proposed that every finite-domain Constraint Satisfaction Problem (CSP) is either in P or it is NP-complete, has been solved independently by Bulatov and Zhuk almost ten years ago. Bodirsky-Pinsker conjecture which states a similar dichotomy for countably infinite first-order reducts of finitely bounded homogeneous structures is wide open. In this paper, we prove that CSPs over first-order expansions of finitely bounded homogeneous model-complete cores are either first-order definable (and hence in non-uniform AC$^0$) or L-hard under first-order reduction. It is arguably the most general complexity dichotomy when it comes to the scope of structures within Bodirsky-Pinsker conjecture. Our strategy is that we first give a new proof of Larose-Tesson theorem, which provides a similar dichotomy over finite structures, and then generalize that new proof to infinite structures.

==> chapters/04-infinite/findual.tex <==
\subsection{Equality-free and unbalanced structures}
We will say that a first-order expansion $\sA$ of a finitely bounded homogeneous structure is
\emph{equality-free} if $=_A(x,y) \equiv (x = y \wedge A(x) \wedge A(y))$, where $A$ is an unary orbit with $|A| \geq 2$, is not \efpp-definable. We say that $\sA$ is \emph{unbalanced} when there is no stable, balanced, and proper implication in $\sA$. The goal now is to show that
an equality-free and unbalanced $\sA$ has finite duality. We take steps analogous to what we did in the previous section for finite structures.

A version of the following lemma is Lemma~20 in~\cite{NagyPW-jonsson}.

\begin{lemma}\label{lemma:core-bwidth}
Let $k, \ell \geq 1$ and  $\sB$ be a $k$-homogeneous $\ell$-bounded model-complete core and $\sA$ be an unbalanced and equality-free first-order expansion of $\sB$.
Let $\instance =(\V,\constraints)$ be a nontrivial, $(k,\max(k, \ell))$-minimal instance of $\csp(\sA)$ such that for every $\tuple v\in I^{\V}_k$, $\proj_{\tuple v}(\instance)$ contains precisely one almost injective 
orbit of $k$-tuples in $\sB$. Then $\instance$ has a solution.
\end{lemma}
\begin{proof}
Observe first that since $\sA$ is $k$-homogeneous and $\instance$ is $(k,\max(k,\ell))$-minimal and nontrivial, every constraint in $\instance$ contains precisely one orbit. 
Also, notice that since $\sA$ is equality-free, this is an almost injective orbit.
Let $\instance'$  be an extension of $\instance$ 
which additionally contains a constraint $C_{\tuple v} = \{ f \mid f \in \proj_{\tuple v}(\instance) \}$  for every tuple of at most $k$ pairwise different variables. Since $\sB$ is $k$-homogeneous and $\ell$-bounded, we have that $\instance'$ is an instance of $\csp(\sA)$ by the assumption from Section~\ref{assum:a-cont-efpp} that $\sA$ as a model-complete core and an expansion of a $k$-homogeneous $\ell$-bounded structure contains all almost injective orbits of at most $\max(k, \ell,\text{arity}(\sA))$-tuples. Then for every one element set $C$ definable in $\sA$ we identify all variables $y$ in $\instance'$
such that $\proj_{(y)} (\instance)$ is a constraint over $C$. The identification involves replacing constraints with new ones in which several identified variables are replaced by a single variable, and the mappings in the constraints are altered accordingly. Observe that now every constraint is over exactly one injective orbit.
Name this new instance $\instance ''$. It is also an instance of $\csp(\sA)$. 
Consider now an instance $\instance''_B$ which is a restriction of $\instance''$ to the constraints that correspond to relations which are actually in $\sB$. In particular, this instance contains all constraints $C_{\tuple v}$ introduced above. By the $k$-homogeneity of $\sB$, it follows that $\instance''_B$ has a solution if and only if $\instance$ has a solution.

In order to show the former, consider the structure $\sD_B$ over the domain $\V$ which for every $R$ in the signature $\tau_{\sB}$ of $\sB$ contains a tuple $\tuple v$ if and only if there is a constraint $C_{\tuple v}$ in $\instance''_B$ with the scope $S(\tuple v)$ such that  $\{ f(\tuple v) \mid f \in C_{\tuple v} \} = R^{\sB}$.
We claim that $\sD_B$ embeds into $\sB$. Suppose, for contradiction, that it is not the case. Then there exists a bound $\sF$ of size $b$ with $b\leq \ell$ such that $\sF$ embeds into $\sD_B$ via $g$. Let $v_1,\ldots,v_b$ be all elements in the image of this embedding. Find a constraint $C\in \instance$ such that $v_1,\ldots,v_b$ are contained in its scope.
Since $C$ is non-empty, there exists $f\in C$ which, by the observation above, is injective. 
Further, the composition of $g$ and $f$ is an embedding of  $\sF$ into $\sB$, which yields a contradiction. Now, the embedding of $\sD_B$  into $\sB$ is a solution of $\instance''_B$. It completes the proof of the lemma.
\end{proof}


We now turn to proving that every unbalanced and equality-free $\sA$ has relational width $(k, \max(k,\ell))$. The following proposition is a generalization of Proposition~21 in~\cite{NagyPW-jonsson}.

\begin{proposition}\label{prop:widthunbalanced}
Let $k,\ell \geq 1$ and $\sB$ be a $k$-homogeneous $\ell$-bounded model-complete core and $\sA$ be an unbalanced and equality-free first-order expansion of $\sB$.
Then $\sA$ has relational width $(k,\max(k, \ell))$.
\end{proposition}
\begin{proof}
Let $\instance=(\V,\constraints)$ be a non-trivial $(k,\max(k, \ell))$-minimal instance of $\csp(\sA)$; we will show that there exists a solution to $\instance$.
To this end, we will inductively define, for every $i\geq 0$, a $(k,\max(k, \ell))$-minimal instance $\instance_i=(\V,\constraints_i)$ of $\csp(\sA)$ with the same variable set as $\instance$ such that $\instance_0=\instance$ and such that for every $i\geq 1$, $\constraints_i$ contains for every constraint $C_{i-1}\in\constraints_{i-1}$ a constraint $C_i$ such that $C_i\subseteq C_{i-1}$, and such that moreover for some $\tuple v_i \in I^{\V}_m$ with $m \leq k$, it holds that $\proj_{\tuple v_i}(\instance_i) \subsetneq \proj_{\tuple v_i}(\instance_{i-1})$, or for every $\tuple v\in I^{\V}_k$, it holds that $\proj_{\tuple v}(\instance_i)$ contains only one almost injective orbit in $\sB$.


Let $\instance_0:=\instance$. Let $i\geq 1$. We define $\mathcal{G}_i$ to be the digraph over
vertices of the form $(C,\tuple v)$ where  $\tuple{v}$ is a tuple of pairwise different variables of
length $m \leq k$ and $C \subsetneq \proj_{\tuple v} (\instance_{i-1})$ is \efpp-definable in $\sA$.
We have an arc 
$(C,\tuple v) \to (D,\tuple w)$  in $\mathcal{G}_i$ if there is a proper and nontrivial
$(C,\tuple v, D,\tuple w)$-implication $\phi$ in $\sA$ with $\proj_{\tuple x} \phi^{\sA} = \proj_{\tuple x} (\instance_{i-1})$ for all $\tuple x \in \{ \tuple v, \tuple w\}$.

We now claim that under the assumptions of the lemma, either for every $\tuple v\in I^{\V}_k$ the projection $\proj_{\tuple v}(\instance_i)$ contains only one almost injective orbit in $\sB$, and we can invoke Lemma~\ref{lemma:core-bwidth}, or there is $\tuple v\in I^{\V}_m$ for some $m \leq k$ such that $O \subsetneq \{ f(\tuple v) \mid f \in \proj_{\tup v}(\instance_i) \}$ for some almost injective orbit $O$, and, by Observation~\ref{obs:core}, $\mathcal{G}_i$ contains at least one vertex. Indeed, otherwise there exist two variables $u_1, u_2 \in \V$ such that $\proj_{(u_1, u_2)} (\instance_{i-1})$ is a union of orbits of the form 
$=_A(x,y) \equiv A(x) \wedge A(y) \wedge x = y$ with $|A| \geq 2$. If the union is trivial, that is, it consists of only one such $=_A$, then we have a contradiction with the fact that $\sA$ is equality-free. If the union is nontrivial, that is $\proj_{(u_1, u_2)} (\instance_{i-1})$ contains both  
$=_A(x,y)$ as well as some
$=_B(x,y) \equiv B(x) \wedge B(y) \wedge x = y$ with $|B| \geq 2$, then $R_C(x,y)$ such that $R_C = \{ f(u_1, u_2) \mid f \in \proj_{(u_1, u_2)} (\instance_{i-1}) \}$ is a balanced, proper and non-trivial $(A,x, A, y)$-implication. The latter contradicts the assumption that $\sA$ is unbalanced. From now on, we assume that $\mathcal{G}_i$ has at least one vertex. 


\bigskip
\setcounter{claim}{0}
\begin{claim}
For every $i$, the graph $\mathcal{G}_i$ is acyclic. 
\end{claim}

\begin{proof}
Assume, on the contrary, that $\mathcal{G}_i$ contains a cycle. Then there exists $n \in \mathbb{N}$, a proper and nontrivial $(C_i, \tuple x_i, C_{i_1}, \tuple x_{i+1})$-imp\-li\-ca\-tion $\psi_i$ in $\sA$ for all  $i \in [n-1]$ as well as a $(C_n, \tuple x_n, C_1, \tuple x_1)$-implication $\psi_n$ in $\sA$. Rename the variables $\tuple x_1$ in $\psi_n$ to $\tuple x_{n+1}$ so that the obtained implication $\phi'$ was a $(C_n, \tuple x_n, C_1, \tuple x_{n+1})$-implication. By Lemma~\ref{lemma:implcomp}, it follows that $\phi := \psi_1 \circ \cdots \circ \psi_{n-1} \circ \phi'$ is a non-trivial, proper and balanced $(C_1, \tuple x_1, C_1, \tuple x_{n+1})$-implication. By Lemma~\ref{lem:obtainingstable}, we may obtain from $\phi$ a stable, proper and balanced implication in $\sA$ which contradicts the fact that $\sA$ is unbalanced.
\end{proof}

 
 By the claim above, the graph $\mathcal{G}_i$ has a sink $(F_{\tuple v_i},\tuple v_i)$ in $\mathcal{G}_i$ for some $\tuple v_i \in I^{\V}_m$ with $m \leq k$.  We intend to choose a sink in $\mathcal{G}_i$ with an additional property.
 We say that $(F_{\tuple v_i}, \tuple v_i)$ is \emph{simplified} if
 for every $\tuple w_i$ with $\scope(\tuple w_i) \subsetneq \scope(\tuple v_i)$ it holds that  
 $\proj_{\tuple w_i} (F_{\tuple v_i}(\tuple v_i))^{\sA} = \proj_{\tuple w_i}(\instance_{i-1})$.

 \bigskip
 \begin{claim}
 There exists a sink $(F_{\tuple v_i},\tuple v_i)$ in $\mathcal{G}_i$ which is simplified.   
 \end{claim}
 

\begin{proof}
Observe first that if $(F_{\tuple v_i},\tuple v_i)$ is not  \emph{simplified} because 
$(\proj_{\tuple w_i} (F_{\tuple v_i}(\tuple v_i))^{\sA} \neq \proj_{\tuple w_i}(\instance_{i-1}))$ for some subtuple $\tuple w_i$ of $\tuple v_i$, then the pair $(\proj_{\tuple w_i} (F_{\tuple v_i}(\tuple v_i))^{\sA},\tuple w_i)$
is a vertex in $\mathcal{G}_i$. In particular, there is a subtuple $\tuple w_i$ of $\tuple v_i$ such that $(\proj_{\tuple w_i} (F_{\tuple v_i}(\tuple v_i))^{\sA},\tuple w_i)$ is simplified. In the worst case, $\tuple w_i$ contains only one variable.

Choose therefore some simplified vertex $(D_1, \tuple w_1)$  in $\mathcal{G}_i$. Either it is a sink or there is some non-trivial and proper $(D_1, \tuple w_1, D_2, \tuple w_2)$-implication $\phi$ in $\sA$. We claim that in the latter case, we can choose $( D_2, \tuple w_2)$, which is simplified. Indeed, suppose $(D_2, \tuple w_2)$ is not simplified and $(D_2, \tuple w_2)$ is a pair with the shortest $\tuple w_2$ so that such an implication $\phi$  in $\sA$ exists. 
Then, there exists $\tuple x$ with $\scope(\tuple x) \subsetneq \scope(\tuple w_2)$ such that $\proj_{\tuple x} (D_2(\tuple w_2))^{\sA} \neq \proj_{\tuple x}(\instance_{i-1})$. Since $\phi$ is proper we have that $\scope(\tuple x)$ is not contained in $\scope(\tuple w_1) \cap \scope(\tuple w_2)$. It follows that $\phi$ is also a proper and non-trivial $(D_1, \tuple w_1,  \proj_{\tuple x}(D_2(\tuple w_2))^{\sA}, \tuple x)$-implication. Since $\tuple x$ is shorter than $\tuple w_2$ we have the contradiction and we can assume  that $(D_2, \tuple w_2)$ is simplified. In the same fashion, we can choose
$( D_3, \tuple w_3), \ldots, ( D_m, \tuple w_m)$ which are all simplified and such that for every $i \in [m-1]$ there is a $(D_i, \tuple w_i, D_{i+1},  \tuple w_{i+1})$-implication $\phi$ in $\sA$ with $\proj_{\tuple z}(\phi_i^{\sA}) = \proj_{\tuple z} (\instance_{i-1})$ for all $\tuple z \in \{ \tuple w_i, \tuple w_{i+1} \}$. It follows that $\mathcal{G}_i$ 
contains a path $(D_1, \tuple w_1) \to \cdots \to (D_m, \tuple w_m)$. Since $\mathcal G_i$ is acyclic, with $m$ large enough we may conclude that $(D_m, \tuple w_m)$ is a desired simplified sink in $\mathcal{G}_i$.
\end{proof}


 
 In order to define $\instance_{i}$ we set 
 $C_i := \{f \in C_{i-1}\mid  f(\tuple v_i) \in F_{\tuple v_i} \}$ when the scope of $C_i$ contains $\scope(\tuple v_i)$ and $C_i := C_{i-1}$ otherwise.
Clearly, $C_i\subseteq C_{i-1}$.
Finally, we define $\constraints_{i}=\{C_{i}\mid C_{i-1}\in\constraints_{i-1}\}$. Observe that the following claim completes the proof of the proposition.

\bigskip
\begin{claim}\label{claim:projs}
Assume that $\mathcal G_i$ is acyclic. Then, for every $i\geq 1$, the instance $\instance_i$, as defined above, is a nontrivial and $(k, \max(k, \ell))$-minimal instance of $\csp(\sA)$. Moreover, for every $\tuple v \in I^{\V}_m$ with $m \leq k$ and $\scope(\tuple v_i) \subseteq \scope(\tuple v)$ we have $\proj_{\tuple v}(\instance_{i}) = \{ f \mid f \in \proj_{\tuple v}(\instance_{i-1})  \wedge f(\tuple v_i) \in F_{\tuple v_i} \}$ and  $\proj_{\tuple v}(\instance_{i}) = \proj_{\tuple v}(\instance_{i-1})$ otherwise.
\end{claim}

\begin{proof}
The instance $\instance_i$ is nontrivial since $\instance_{i-1}$ is $(k, \max(k,l))$-minimal.

To show that $\instance_i$ is $(k, \max(k,l))$-minimal and that the projections of $\instance_i$ to tuples of at most $k$ variables are as in the formulation of the claim, assume on the contrary that there is a constraint $C_i$ whose scope contains $\tuple v$ of length at most $k$ and $\proj_{\tuple v} (C_i)$ is not as desired. 
Observe first that by $(k, \max(k,\ell))$-minimality of $\instance_{i-1}$ we have that $\scope(\tuple v)$ cannot contain $\scope(\tuple v_i)$. However, by the construction of $\instance_{i}$, the scope of $C_i$ contains $\tuple v_i$.
It follows that the desired value of $\proj_{\tuple v} (C_i)$ is $\proj_{\tuple v}(\instance_{i-1}) = \proj_{\tuple v} (C_{i-1})$. Since it is not the case, we have that  $R_{C_{i-1}}(\tuple x)$ where $\scope(\tuple x)$ is the scope of $C_{i-1}$ and $R_{C_{i-1}} = \{ f(\tuple x) \mid f \in C_{i-1} \}$ 
is a $(F_{\tuple v_i}, \tuple v_i, F_{\tuple v}, \tuple{v})$-implication for some $F_{\tuple v} \subsetneq \proj_{\tuple v} (R_{C_{i-1}}(\tuple x))^{\sA}$.
Since $(F_{\tuple v_i}, \tuple v_i)$
is simplified, we have that $\scope(\tuple v)$ cannot be contained in $\scope(\tuple v_i)$. Hence $\scope(\tuple v_i)$ is not comparable with $\scope(\tuple v)$ w.r.t. the inclusion. It follows that $\phi$ is non-trivial. It is also proper since $(F_{\tuple v_i}, \tuple v_i)$ is simplified. 
Thus, the existence of $\phi$ contradicts the fact $(F_{\tuple v_i}, \tuple v_i)$ is a sink in $\mathcal{G}_i$. It completes the proof of the fact that $\instance_i$ is $(k,\max(k,l))$-minimal. 

By the assumption in Section~\ref{sect:prelim}, all \efpp-definable relations of arity up to $\max(k, \ell,\text{arity}(\sA))$ are in $\sA$; it follows that $\instance_i$ is an instance of $\csp(\sA)$.
\end{proof}

\end{proof}


\subsection{Rewriting \texorpdfstring{$(k,\max(k,l))$}{(k,max(k,l))}-minimality}

Let $k,l \geq 1$ and $\sA$ be a first-order expansion of a $k$-homogeneous $l$-bounded model-complete core $\sB$ and $\instance = (\V, \constraints)$ be an instance of $\csp(\sA)$. We define $\instance_{\max} = (\V, \constraints_{\max})$ so that $\constraints_{\max}$ contains $\constraints$ and additionally all constraints $A^U$ for all $\max(k,l)$-element subsets $U$ of $\V$. Algorithm~\ref{alg2:cap} presented below 
enforces the second condition in the definition of a $(k,\max(k,l))$-minimal instance working over $\instance_{\max}$. 
It first  updates iteratively the collection of constraints $\mathcal{D}^{\V}_k(\instance) = \{ D_U \mid U  \in \bigcup_{i=1}^k     
\binom{\V}{i} \}$ and then updates $\instance_{\max}$ so that the projections of constraints in new $\constraints_{\max}$ to sets of at most $k$-variables were equal to the constraints in $\mathcal{D}^{\V}_k(\instance)$. 


\begin{algorithm}
\caption{\ \ Let $\sA$ be a first-order expansion of a $k$-homogeneous $l$-bounded model-complete core and $\instance_{\max} = (\V, \constraints_{\max})$ an extension of an instance $\instance = (\V, \constraints)$ of $\csp(\sA)$ such that $\constraints_{\max}$ contains $\constraints$ and additionally all constraints $A^U$ over all $\max(k,l)$-element subsets $U$ of $\V$.}\label{alg2:cap}
\begin{algorithmic}[1]
\ForAll {$U \in \bigcup_{i=1}^k \binom{\V}{i}$} \Comment{Step 1: Initialization}
\label{alg2list:step1}
    \State $D_U \gets A^U$
\EndFor
\\
\While{true} \Comment{Step 2: Pruning}
\label{alg2list:step2}
    \State For some $C \subseteq A^U$ in $\constraints_{\max}$,
and $T \in \bigcup_{i=1}^k \binom{U}{i}$ set:
    \State $\widehat{D_T} \gets \{ f \in A^U \mid \exists g \in C: (f = g|_T) \wedge \bigwedge_{Z \in \bigcup_{i=1}^k \binom{U}{i}} (g|_Z \in D_{Z}) \}$
    \If {for all $C,  T$, their $\widehat{D_T}$ contains $D_T$}
        \State \textbf{break}
    \Else
        \State $D_T \gets D_T \cap \widehat{D_{T}}$
    \EndIf
\EndWhile

\\

\State \textbf{return} $\mathcal{D}_k^{\V}(\instance)$
\Comment{Step 3: Return}
\end{algorithmic}
\end{algorithm}


The goal of the next proposition is to show that the outcome of Algorithm~\ref{alg2:cap} induces on $\instance_{\max}$ a $(k, \max(k,l))$-minimal instance of $\csp(\sA)$. It is a generalization of Proposition~\ref{prop:minAlg1}.

\begin{proposition}
\label{prop:minAlg2}
Let $k,\ell \geq 1$ and $\sA$ be a first-order expansion of a $k$-ho\-mo\-ge\-neous $\ell$-bounded model-complete core,
$\mathcal{I} = (\V, \constraints)$ be an instance of $\csp(\sA)$, and $\instance_{\max} = (\V, \constraints_{\max})$ an extension of  $\instance$  such that $\constraints_{\max}$ contains $\constraints$ and additionally all constraints $A^U$ over all $\max(k,\ell)$-element subsets $U$ of $\V$. 
Then $\mathcal{I}'_{\max} = (\V, \constraints'_{\max})$ obtained from $\mathcal{I}_{\max}$ by replacing every $C \subseteq A^U$ with $$C' = \{ f \in C \mid \bigwedge_{Z \in \bigcup_{i=1}^k \binom{U}{i}} f|_Z  \in  D_Z \}$$ is $(k,\max(k,\ell))$-minimal and equivalent to $\mathcal{I}$.
\end{proposition}
\begin{proof}
To see that $\mathcal{I}'_{\max}$ is equivalent to $\mathcal{I}$, it is enough to observe that whenever Algorithm~\ref{alg2:cap} reduces the set $D_{T}$ for some  $T \in \bigcup_{i \in [k]} \binom{\V}{i} $, the removed values cannot be a part of a solution of $\instance$.

To prove $(k,\max(k,l))$-minimality of $\instance'_{\max}$ assume the contrary. Then, there exists a constraint $C$ of the scope $U$ and $T \in \bigcup_{i=1}^k \binom{U}{i}$  
such that
$$\{ f \in A^T \mid \exists g \in C~(f = g|_T) \wedge \bigwedge_{Z \in \bigcup_{i=1}^k \binom{U}{i}} (g|_Z \in D_{Z}) \}$$ does not contain $D_T$. Because of Step~2, it contradicts the fact that the run of Algorithm~\ref{alg2:cap} over $\instance_{\max}$ is completed and proves the proposition.
\end{proof}

We will now define $k$-tree \efpp-formulae. To this end,
let $\mathcal{I} = (\V, \constraints)$ be an instance of $\csp(\sA)$ and $\mathcal{X}$ be a set of copies of variables from $\V$ such that every its element has infinitely many copies in $\mathcal{X}$. We say that $\tuple x$ is a copy of $\tuple u$, both of length $m$, if  $x_i$ is a copy of $u_i$ for all $i \in [m]$.  
We say that a constraint $C'$ is a copy of a constraint $C \in \constraints$
if it is obtained from $C$ by replacing every variable from $\scope(C)$ by its copy in $\mathcal{X}$. We will also say that an atom $R(\tuple x)$ is a copy of
a constraint $C \in \constraints$ if there exists a constraint $C'$ with the scope $\scope(\tuple{x})$ which is a copy of $C$ and $R = \{ f(\tuple x)  \mid f \in C'  \}$.

\begin{definition}
\label{def:ktree}
Let $\mathcal{I} = (\V, \constraints)$ be an instance of $\csp(\sA)$, 
$\instance_{\max}$ as defined above,  and  $\mathcal{X}$ a set containing infinitely many copies of every variable in $\V$. Let $k \geq 1$,
a \emph{$k$-tree \efpp-formula $\phi$ over  $\mathcal{I}$} with a distinguished tuple $\tuple{r_0}$ of at most $k$ pairwise different variables  in $\text{Var}(\phi)$, called a \emph{root}, is a conjunction of copies of constraints in $\mathcal{C}_{\max}$ 
and is in one of the following forms. 

\begin{enumerate}
\item \label{ktree:1} It is a single atom $R(\tuple{x})$ with $\scope(\tuple r_0) \subseteq \scope(\tuple x)$.

\item \label{ktree:2} It is a conjunction of $k$-tree \efpp-formulae $\phi_1, \ldots, \phi_m$ 
with the roots   $\tuple{r_1}, \ldots, \tuple{r_m}$ and a new copy $\phi_0 := R(\tuple x)$  of a constraint in $\constraints_{\max}$ such that 
\begin{enumerate}
\item \label{ktree:rootsinx} $\bigcup_{i \in \{0, \ldots, m \}}  \scope(\tuple r_i) \subseteq \scope(\tuple x)$, 
\item \label{ktree:onlyroots} $\Var(\phi_0) \cap \Var(\phi_i) =  \scope(\tuple r_i) $ for all $i \in [m]$, and 
\item \label{ktree:rootsinter} $\Var(\phi_i) \cap \Var(\phi_j) =  \scope(\tuple r_i)  \cap \scope(\tuple r_j)$ for all $i,j \in [m]$.
\end{enumerate}
\end{enumerate}

Furthermore, the subformulae $\phi_1, \ldots, \phi_m$ of $\phi$ in Item~\ref{ktree:2} will be called the \emph{leaf subformulae} of $\phi$ and $\phi_0$ the \emph{root subformula} of $\phi$.
A \emph{formula path} in $\phi$ is a sequence  $\psi_1, \ldots, \psi_{t+1}$ of subformulae of $\phi$ such that $\psi_{t+1}$ is $\phi$, $\psi_1$ is an atomic formula and  for every $i \in [t]$,
$\psi_i$ is a leaf subformula of $\psi_{i+1}$.

A $k$-tree \efpp-formula is a $k$-tree \efpp-formula over $\instance$ for some instance $\instance$ of $\csp(\sA)$.
\end{definition}

\noindent
Observe that for every $k$, a $k$-tree \efpp-formula $\phi$ over $\instance$ is quantifier-free.

\begin{definition}
\label{def:inf_ranked_definition}
We say that a $k$-tree \efpp-formula $\phi$ with the root $\tuple r_0$ is a \emph{minimal $k$-tree \efpp-formula over $\instance$} if $\proj_{\tuple r} \phi^{\sA} = B$ and $\phi$ is minimal with respect to the number of atoms among all $k$-tree \efpp-formulae $\psi$ over $\instance$   with the same root $r$ satisfying 
$\proj_{\tuple r} \psi^A = B$.
\end{definition}


Note that in the above definition, we allow $B$ to be equal to $\emptyset$.
The next step is to prove that whenever Algorithm~\ref{alg2:cap} derives some constraint $D_T$
then there is a $k$-tree \efpp-formula $\phi$ whose projection onto its root is the relation corresponding to $D_T$.

\begin{proposition}
\label{prop:Alg2TreeDef}
Let $k, \ell \geq 1$ and $\instance$ be an instance of $\csp(\sA)$ over a first-order expansion of a $k$-homogeneous $\ell$-bounded model-complete core. It follows that whenever Algorithm~\ref{alg2:cap} computes $D_{T}$ with $T = \scope(\tuple t)$ either in Step~1 or Step~2, then there exists a $k$-tree \efpp-formula with the root $\tuple r$ which is a copy of $\tuple t$ in $\mathcal{X}$ such that  $\proj_{\tuple r} \phi^{\sA} = \{ f(\tuple{t}) \mid f \in D_T \}$.
\end{proposition}
\begin{proof}
The proof goes by the induction of the number of steps
executed by Algorithm~\ref{alg2:cap}. For any $D_U$ computed in Step 1, we just take a copy $R(\tuple x)$ of the appropriate full constraint and set the root to $\tuple{x}$.

Assume now that Algorithm~\ref{alg2:cap} computes $D_{T}$ in Step~2 from a constraint $C \subseteq A^U$ in $\constraints_{\max}$. Assume moreover that
$\bigcup_{i \in [k]} \binom{U}{k} = \{ \scope(\tuple z_1), \ldots, \scope(\tuple z_m) \}$
where $m = \sum^k_{i=1}\binom{|U|}{i}$ and $\tuple z_1, \ldots, \tuple z_m$ are tuples of elements in $U$. By the induction hypothesis there are $k$-tree \efpp-formulae $\phi_1, \ldots, \phi_m$ over the roots $\tuple r_1, \ldots, \tuple r_m$ which are copies of $\tuple z_1, \ldots, \tuple z_m$ in $\mathcal{X}$ such that for all $i \in [m]$ the projection of $\phi_i^{\sA}$ onto $\tuple r_i$ is $\{ f(\tuple z_i) \mid f \in D_{\scope(\tuple z_i)} \}$. Let $R(\tuple x)$ be a copy of the constraint $C$ such that $\bigcup_{i \in [m]} \scope(\tuple r_i) \subseteq \scope(\tuple x)$.
Since $\mathcal{X}$ is infinite we may secure
conditions in Items~\ref{ktree:rootsinx}--\ref{ktree:rootsinter} in Definition~\ref{def:ktree}. It is straightforward to check that the  conjunction $\psi$ of $\phi_1, \ldots, \phi_{m}$ and $R(\tuple x)$  seen as a $k$-tree \efpp-formula with the root $\tuple{r_j}$ satisfying $j \in [m]$ and $\scope(\tuple z_j) = T$ is the desired $k$-tree \efpp-formula. Indeed, we have that 
$\proj_{\tuple r_j} \psi^{\sA} = \{ f(\tuple{z_j}) \mid f \in D_{T} \}$.
\end{proof}



The final step is to show that an unbalanced and equality-free $\sA$ has finite duality. However, this step is more complicated for infinite $\sA$ than for finite. We need the following two auxiliary lemmata. 

\begin{lemma}
\label{lem:same-intersection}
Let $k,\ell \geq 1$ and $\sA$ be a first-order expansion of a $k$-homogeneous $\ell$-bounded model-complete core which is also both unbalanced and equality-free.
Let $Z \in \mathbb{N}$, $\phi$ be a $k$-tree \efpp-formula with a formula path containing at least $Z^k$
formulae $\psi_1, \ldots, \psi_{Z^k}$ with roots $\tuple r_1, \ldots, \tuple r_{Z^k}$ such that for all $i \in [Z^k-1]$, $\psi_i$ is a leaf subformula of $\psi_{i+1}$ and $\bigcap_{i \in [Z^k]} \scope(\tuple r_i) \neq \emptyset$. Then there exists $\tuple p_1, \ldots, \tuple p_{Z} \in \{ \tuple r_1, \ldots, \tuple r_{Z^k} \}$
and 
$\tuple z$ of length at most $k$ satisfying $\scope(\tuple z) = \scope(\tuple p_i) \cap \scope(\tuple p_j)$ for all $i,j \in [Z]$.
\end{lemma}


\begin{proof}
Observe first that by Item~\ref{ktree:onlyroots} in Definition~\ref{def:ktree}, we have $\scope(\tuple
r_i) \cap \scope(\tuple r_{i+1}) \supseteq \scope(\tuple r_i) \cap \scope(\tuple r_{i+2})$ for all $i \in [Z^k-2]$. 
It generalizes to $\scope(\tuple r_i) \cap \scope(\tuple r_{j_1}) \supseteq \scope(\tuple r_i) \cap \scope(\tuple r_{j_2})$ for all
$i < j_1 < j_2$ in $[Z^k]$.
In particular, we have that if $\scope(\tuple r_{j_1}) \cap \scope(\tuple r_{j_2}) = S$ and
$\scope(\tuple r_{j_2}) \cap \scope(\tuple r_{j_3}) = S$, then $\scope(\tuple r_{j_1}) \cap \scope(\tuple r_{j_3}) = S$  for all $j_1 < j_2 < j_3$ in $[Z^k]$.


Let now $\tuple x$ be such that $\bigcap_{i \in [Z^k]} \scope(\tuple r_i) = \scope(\tuple x)$ and consider a maximal sequence $i_1 = 1 < \cdots < i_T \leq Z^k$ constructed so that for every $j \in [T-1]$ the index $i_{j+1}$ is the smallest larger than $i_j$ such that $\scope(\tuple r_{i_j}) \cap \scope(\tuple r_{i_{j+1}}) = \scope(\tuple x)$. 
By the observation above, it holds $\scope(\tuple r_{i_{j_1}}) \cap \scope(\tuple r_{i_{j_2}}) = \scope(\tuple x)$
for all $j_1, j_2 \in [T]$. Now, either $T \geq Z$ and  we are done or there exists $j \in T$ such
that $i_{j+1} - i_{j} \geq (Z)^{k-1}$. By the construction of the sequence and the observation above
we have that there exists $\tuple x'$ with  $\scope(\tuple x') \supsetneq \scope(\tuple x)$ such that
$\bigcap_{m \in [i_{j}, i_{j+1})} \scope(\tuple r_m) = \scope(\tuple x')$. Now, either $|\scope(\tuple x')| = k$ and we are done or we repeat the above reasoning with $\tuple x'$ instead of $\tuple x$. Since the size of a root in a $k$-tree \efpp-formula is at most $k$, the above reasoning repeated at most $(k-1)$ times gives us the desired set of roots $\{\tuple p_1, \ldots, \tuple p_Z \}$.
\end{proof}

\noindent
We now turn to the second auxiliary lemma. 

\begin{lemma}
\label{lem:nonempty-intersection}
Let $k, \ell \geq 1$ and $\sA$ be an unbalanced 
first-order expansion of a $k$-homogeneous $\ell$-bounded  model-complete core $\sB$ such that there are exactly $K$ pairwise different orbits of $k$-tuples in $\sB$ and let $L = 2^K$ be the number of all $k$-ary first-order definable relations in $\sB$. 

Let $\phi$ be a minimal $k$-tree \efpp-formula such that the projection of $\phi^{\sA}$ onto its root is nonempty, and let $\pi$ be a formula path in $\phi$. Then $\pi$ contains less than $P = (K \cdot (L^2 \cdot k + 3))^k$ formulae $\psi'_1, \ldots, \psi'_P$ with the roots $\tuple r_1, \ldots, \tuple r_P$ such that $\bigcap_{i \in [P]} \scope(\tuple r_i) \neq \emptyset$. 
\end{lemma}



\begin{proof}
Assume, on the contrary, that there is such a formula path in $\phi$ which contains at least $P$ formulae $\psi'_1, \ldots, \psi'_P$ satisfying the condition from the formulation of the lemma.
By Item~\ref{ktree:onlyroots} in Definition~\ref{def:ktree}, we may assume that $\psi'_1, \ldots, \psi'_P$ are consecutive in $\pi$, that is, $\psi'_i$ is a leaf subformula of $\psi'_{i+1}$ for all $i \in [P-1]$.
By Lemma~\ref{lem:same-intersection}, the formula path $\pi$ contains at least $Z = K \cdot( L^2 \cdot k + 3)$ pairwise different $k$-tree \efpp-subformulae $\psi_1, \ldots, \psi_Z$ with roots $\tuple p_1, \ldots \tuple p_Z$  such that $\psi_i$ is a subformula of $\psi_{i+1}$ for all $i \in [Z-1]$ and $\scope(\tuple z) = \scope(\tuple p_i) \cap \scope(\tuple p_j)$ for all $i,j \in [Z]$ and some tuple $\tuple z$ of at most $k$ pairwise different variables in $\mathcal{X}$.    


For all $i \in [Z]$, set now
$D_i := \proj_{\tuple z} (\psi_i)^{\sA}$. It follows that $D_1 \supseteq \cdots \supseteq D_Z$ since for all $i \in [Z-1]$, $\psi_i$ is a subformula of $\psi_{i+1}$.
Furthermore, since there are at most $K$ different orbits of $k$-tuples in $\sB$, there are at most $K$ pairwise different values in the sequence above. 
By the choice of $Z$, there exists $i \in [Z]$ so that
$D_i = \cdots = D_{i + L^2 \cdot k + 2}$. Set $j := i + L^2 \cdot k + 2$.
Since $\phi$ is minimal, then also $\psi_j$ is minimal.

Let now $\zeta'_i$ be a copy of $\psi_i$ with the variables renamed so that the only variables contained both in $\zeta'_i$ and $\psi_{j}$ are the variables in $\tuple z$ and let $\zeta_i$ be a $k$-tree \efpp-formula created from $\zeta'_i$ by perhaps removing certain variables from the root of $\zeta'_i$ so that the root of the new formula $\zeta_i$ was just $\tuple z$. This perhaps new root is the only difference between $\zeta_i$ and $\zeta'_i$.
Then, assume without loss of generality that
$\psi_{j}$ consists of a root subformula $R(\tuple x)$
and leaf subformulae $\xi_1, \ldots, \xi_o$. Construct  $\theta_{j}$ according to the recipe in Item~\ref{ktree:2} in Definition~\ref{def:ktree} out of $R(\tuple x)$ as a root subformula and $\xi_1, \ldots, \xi_o$ but also $\zeta_i$ as its leaf-subformulae. By the choice of $i$ and the construction of $\zeta_i$, it follows that the projection of both $(\zeta_i)^{\sA}$ and $(\psi_{j})^{\sA}$, and in consequence of $(\theta_{j})^{\sA}$ onto $\tuple z$ is the same. It follows that the projections of  $(\theta_{j})^{\sA}$ and $(\psi_j)^{\sA}$ onto $\tuple p_j$ are the same. Denote this projection by $C_j$.

Clearly, $\theta_j$ is not minimal. Remove therefore, one by one, atoms from the bottom of $\psi_i$, which is by the construction, a subformula of $\theta_j$, so that the obtained formula was always a $k$-tree \efpp-formula, and
until we obtain a subformula $\theta'_j$ of $\theta_j$ such that the projection $C'_j$ of $(\theta'_j)^{\sA}$ onto $\tuple p_j$ is a non-trivial superset of $C_j$ or until all atoms from $\psi_i$ are removed. Since $\psi_i$ has the same number of atoms as $\zeta_i$, in the latter case, the obtained formula has the same number of atoms as $\psi_j$, and hence it is minimal. Thus, remove one more constraint from $\psi_{i+1}$. Since $|j - i| \geq 3$, observe that the new formula is a $k$-tree \efpp-formula and denote the new formula by $\theta'_j$. By minimality, also in this case, the projection $C'_j$ of $(\theta'_j)^{\sA}$ onto $\tuple p_j$ is a nontrivial superset of $C_j$.
By the construction, the formula $\theta'_j$ may not contain the formula $\psi_{i+1}$ but it contains all $\psi_{i+2}, \ldots, \psi_j$ and hence roots $\tuple p_{i+2}, \ldots, \tuple p_j$.  For all $k \in [i+2,  j]$, denote by $C_k$ and $C'_k$ the projection of $\theta_{j}^{\sA}$ and $(\theta'_{j})^{\sA}$ onto $\tuple p_k$, respectively. Since $C_j \subsetneq C'_j$, by the construction of a $k$-tree \efpp-formula, it follows that $C_k \subsetneq C'_k$ for all $k \in [i+2, j]$. 


Now, by the counting argument, there are $k_1 < k_2$ in $[i+2,j]$ such that $(C_{k_1}, C'_{k_1})$ equals  
$(C_{k_2}, C'_{k_2})$. Denote that pair by $(C, C')$.
It follows that $\theta'_{j}$ is a balanced $(C, \tuple p_{k_1},  C, \tuple p_{k_2} )$-implication with $C' = \proj_{\tuple p_{k_1}} (\theta'_j)^{\sA} = \proj_{\tuple p_{k_2}} (\theta'_j)^{\sA}$.
Since $D_i = \cdots = D_{j}$, by the minimality of $\psi_{j}$, we may assume that $\scope(\tuple z)$ is strictly contained in both $\scope(\tuple p_{k_1})$ and $\scope(\tuple p_{k_2})$, Thus,  $\scope(\tuple p_{k_1})$ and $\scope(\tuple p_{k_2})$ are incomparable with respect to the inclusion, which implies that the implication is nontrivial.   Furthermore, since $\theta'_j$ contains $\zeta_i$, the  projection  of both $(\theta'_{j})^{\sA}$ and
$(\theta_{j})^{\sA}$ to $\tuple z$ is $D_i$. Hence, the implication is proper. 
 By Lemma~\ref{lem:obtainingstable}, the existence of a nontrivial, proper, and balanced implication in $\sA$ contradicts the assumption that $\sA$ is unbalanced and completes the proof of the lemma. 
\end{proof}

\noindent
We are now ready to prove that every unbalanced and equality-free $\sA$ has finite duality.

\begin{proposition}
\label{prop:noimpfindual}
Let $k, \ell \geq 1$ and $\sA$ be a finite-signature first-order expansion of a $k$-homogeneous $\ell$-bounded model-complete core $\sB$. Suppose that $\sA$ is unbalanced and equality-free, then $\sA$ has finite duality.
\end{proposition}

\begin{proof}
By  Propositions~\ref{prop:widthunbalanced}, \ref{prop:minAlg2}, and~\ref{prop:Alg2TreeDef}, for every unsatisfiable instance $\instance$ of $\csp(\sA)$ there is 
a minimal $k$-tree \efpp-formula $\phi_{\instance}$ over $\instance$ such that the projection of $\phi_{\instance}^{\sA}$ is  $\emptyset$. Without loss of generality, we assume that it does not hold for any proper subformula of $\phi_{\instance}$ that is a $k$-tree \efpp-formula.

Let $\Phi'_{\sA}$ be the set of all formulae $\phi_{\instance}$ over all unsatisfiable 
instances $\instance$ of $\csp(\sA)$ and $\Phi_{\sA}$ be a maximal subset of $\Phi'_{\sA}$ such that no two formulae in $\Phi_{\sA}$ may be obtained from each other by renaming the variables.
Assume first that every formula in $\Phi_{\sA}$ has a longest formula path shorter than $M = P \cdot (k \cdot L^2  + 1) +1$  where $P = (K \cdot (L^2\cdot k +3))^k$ is the constant from Lemma~\ref{lem:nonempty-intersection}, $K$ is the number of pairwise different orbits of $k$-tuples in $\sB$ and $L = 2^K$ the number of all $k$-ary first-order definable relations in $\sB$. We will show that in this case $\Phi_{\sA}$ is of finite size.

\bigskip 
\setcounter{claim}{0}
\begin{claim}
Let $i \in \mathbb{N}$. Then there are only finitely many, up to the renaming of variables,  minimal $k$-tree \efpp-formulae with a longest formula path shorter than $i$.
\end{claim}

\begin{proof}
The proof goes by induction on $i$. 
Since the signature of $\sA$ is finite, there are clearly only finitely many different atomic formulae up to the renaming of the variables, and hence finitely many minimal $k$-tree \efpp-formulae with a longest formula path of length $1$. For the induction step, assume that we are done for $i$ and we want to show that there are finitely many, up to the renaming of the variables, minimal $k$-tree \efpp-formulae of a longest formula path shorter than $i+1$. 
 All such $k$-tree \efpp-formulae $\phi$ are formed as in Item~2 of Definition~\ref{def:ktree}. According to the definition, $\phi$
with the root $\tuple r_0$ is formed out of an atomic formula $R(\tuple x)$
and $k$-tree \efpp-formulae $\phi_1, \ldots, \phi_t$. We claim that if $\phi$ is  minimal, then     
$t \leq \sum_{i \in [k]} \left|\binom{\scope(\tuple x)}{i}\right| \cdot K$.
Assume the contrary. Then there exists $\tuple r$ which is a root of $K' > K$ formulae out of $\phi_1, \ldots, \phi_t$. Denote them $\psi_1, \ldots, \psi_{K'}$ and recall from the definition that $\Var(\psi_{j}) \cap \Var(\psi_{j'}) = \scope(\tuple r)$ for any $j, j' \in [K']$.
Since the number of pairwise different orbits of $k$-tuples in $\sB$ is $K$, it follows that there are $\zeta_1, \ldots, \zeta_{K} \subseteq \{ \psi_1, \ldots, \psi_{K'} \}$ such that the projection of $(\bigwedge_{j \in K'} \psi_j)^{\sA}$ onto $\tuple r$ is the same as the projection of $(\bigwedge_{j \in K} \zeta_j)^{\sA}$ onto $\tuple r$. It follows that the projection $(\phi')^{\sA}$ for $\phi'$ obtained from $\phi$ by replacing $\bigwedge_{j \in K'} \psi_j$ with $\bigwedge_{j \in K} \zeta_j$ is the same as the projection of $\phi^{\sA}$ onto $\tuple r$. It contradicts the assumption that $\phi$ is minimal. Thus, a minimal $k$-tree formula $\phi$ with a longest formula path shorter than $i+1$ is built from at most $t = \sum_{i \in [k]} \left|\binom{\scope(\tuple x)}{i} \right| \cdot K$ pairwise different $k$-tree \efpp-formulae of a longest formula path shorter than $i$ and a new single atom. By the induction hypothesis, there are finitely many different, up to the renaming of the variables, of those, and hence finitely many, up to the renaming of variables,  $k$-tree \efpp-formulae of a longest formula path shorter than $i+1$.  
\end{proof}

Let $\phi$ be a $k$-tree \efpp-formula in $\Phi'_{\sA}$. We will write $\phi^*$ for a subformula of $\phi$ which contains only atoms that are copies of constraints in $\instance$.
We write $\sD_{\psi}$ for the canonical structure of an \efpp-formula $\psi$. The domain of $\sD_{\psi}$ is the set of variables in $\psi$  
and $R^{\sD_{\psi}}$ for $R$ in a signature of $\sA$ has a tuple $\tuple{x}$ iff $\psi$ contains an atom $R(\tuple{x})$.

In order to complete the proof of the first case, we will show that 
$\mathcal{O} = \{ \sD_{\phi^*} \mid \phi \in \Phi_{\sA} \}$ is an obstruction set for $\sA$. Assume first that $\instance$ does not have a solution. Then there exists a minimal $k$-tree \efpp-formula $\phi'$ over $\instance$ defining $\emptyset$. The formula $\phi'$ is in $\Phi'_{\sA}$ and its renaming $\phi$ in $\Phi_{\sA}$.
The canonical structure $\sD_{\phi^{*}}$ maps to $\instance$ by first renaming the variables so that the image contained the variables in $\phi'$ and then by taking a homomorphism
which sends every variable in $\phi'$, which is a copy of a variable in $\instance$, to the original variable. On the other hand, the projection of $\phi$ on its root is empty, and hence $\sD_{\phi}$ does not map to $\sA$. Since the only difference between $\phi^*$ and $\phi$ is that the latter formula contains atoms built out of full relations, there is also no homomorphism from $\sD_{\phi^*}$ to $\sA$, and hence if it does map to $\instance$, then it has no solution.

To complete the proof we will show that whenever $\Phi_{\sA}$ contains a minimal $k$-tree \efpp-formula $\phi$ with a formula path $\pi'$ longer than or equal to $M = P \cdot (k \cdot L^2  + 1) +1$, then there is a non-trivial, proper and balanced implication in $\sA$, which contradicts the fact that $\sA$ is unbalanced. 
Let $\psi$ be a leaf subformula of $\phi$ containing $\pi'$ and 
$\pi$ be the restriction of $\pi'$ to $\psi$. By the assumption above, the projection of $\psi^{\sA}$ to its root is non-empty. Furthermore, $\psi$ is minimal since $\phi$ is minimal.  It also holds that the formula path $\pi$ in $\psi$ is longer than or equal to $M-1$ and, in particular, it has roots $\tuple r_{1}, \ldots, \tuple r_{M-1}$ counting from the bottom of $\pi$ to the root subformula of the whole formula. We will now show that the sequence above contains at least $k \cdot L^2 + 1$
roots of pairwise different scope. By Item~\ref{ktree:onlyroots} in Definition~\ref{def:ktree}, for all $i < i_1 < i_2 \leq M-1$  we have that $\scope(\tuple r_i) \cap \scope(\tuple r_{i_1}) \supseteq \scope(\tuple r_i) \cap \scope(\tuple r_{i_2})$. Thus, by Lemma~\ref{lem:nonempty-intersection}, it follows not only that $\bigcap_{i=1}^{P+1} \scope(\tuple r_i) = \emptyset$ but also that $\scope(\tuple r_1) \cap \scope(\tuple r_{P+1}) = \emptyset$.
By the choice of $M$, we have that $\pi$ contains at least $(k \cdot L^2 + 1)$ $k$-tree \efpp-formulae $\psi_1, \ldots, \psi_{k \cdot L^2 + 1}$ with roots $\tuple p_1, \ldots, \tuple p_{k \cdot L^2 + 1}$ of pairwise disjoint scopes. 


Consider now $\psi'$ obtained from $\psi$ by removing an atom from the bottom of $\pi$. Since $\psi$ is minimal, we have that  the projection $C_i$ of $\psi^{\sA}$ to $\tuple p_i$ is strictly contained in the  projection $C'_i$ of
$(\psi')^{\tuple A}$ to $\tuple p_i$ for all $i \in [k \cdot L^2 + 1]$. By the counting argument, there exist $j_1, j_2 \in [k \cdot L^2 + 1]$ such that $(C_{j_1}, C'_{j_1}) = (C_{j_2}, C'_{j_2})$. Denote the pair by $(C, C')$.
It is now easy to see that $\psi'$ is a  balanced $(C,C)$-implication. Since $\scope(\tuple p_{j_1}) \cap \scope(\tuple p_{j_2}) = \emptyset$, the implication is proper and non-trivial. By Lemma~\ref{lem:obtainingstable}, it contradicts the fact that $\sA$ is unbalanced and completes the proof of the proposition. 
\end{proof}

We are now ready to provide the proof of the main theorem of this paper.

\main*

\begin{proof}
Since the signature of $\sB$ is finite, this structure is $k$-homogeneous and $\ell$-bounded for some $k,\ell \in \mathbb{N}$.
If there is an \efpp-definition of a stable, balanced, and proper implication or of equality in $\sA$, then $\csp(\sA)$ is L-hard under first-order reduction by Propositions~\ref{prop:balimpLhard} and~\ref{prop:equalityLhard}, respectively. Otherwise, the structure $\sA$ is called unbalanced and equality-free. By Proposition~\ref{prop:noimpfindual}, it has finite duality. Thus, $\csp(\sA)$ is first-order definable and in nonuniform AC$^0$. It completes the proof of the theorem.
\end{proof}


==> chapters/04-infinite/hardness.tex <==
In this section, we provide hardness results. First, we prove that an expansion of any model-complete core $\sB$ by a balanced implication with some extra reasonable properties gives rise to an $L$-hard CSP.

\begin{proposition}
\label{prop:balimpLhard}
Let $k,l \geq 1$ and $\sA$ be a first-order expansion of a $k$-homo\-ge\-neous $l$-bounded model-complete core $\sB$. Suppose that there is a stable, balanced, and proper $(C, \tuple u, C, \tuple v)$-implication $\phi$  in $\sA$.  Then $\csp(\sA)$ is L-hard under first-order reduction.  
\end{proposition}
\begin{proof}
Let $D:= \proj_{\tuple u} \phi^{\sA} = \proj_{\tuple v } \phi^{\sA}$. We first define
$\mathcal{B}_{\phi}$ to be a directed graph over orbits of tuples in $\sB$ contained in $D$ such that there is an arc
$O \to P$ if $\phi^{\sA}$ contains an OP-mapping. We call a strongly connected component in
$\mathcal{B}_{\phi}$ that has at least one arc a \emph{component}. 
A component $F$ in  $\mathcal{B}_{\phi}$ is a
\emph{sink} in $\mathcal{B}_{\phi}$ if every arc originating in $F$ ends up in $F$. On the other
hand, a component $F$ is a \emph{source} in $\mathcal{B}_{\phi}$ if every arc targeting an element in $F$ starts also in $F$. 

Let $\tuple z$ be such that $\scope(\tuple z) = \scope(\tuple u) \cap \scope(\tuple v)$ and assume that both $\tuple u$ and $\tuple v$ are of length $m \leq k$. Since $\phi$ is stable, we may assume that $\tuple z = (u_{r+1}, \ldots u_m) = (v_{r+1}, \ldots, v_m)$ for some $r \in [m]$. If $r = m$, then we assume that $\scope(\tuple z)$ is empty. Further we assume that all free variables of $\phi(u_1, \ldots, u_r,\allowbreak v_1, \ldots, v_r,\allowbreak v_{r+1}, \ldots, v_m)$ are those mentioned in the brackets.
Since $\phi$ is proper, there exists an orbit $P \in \proj_{\tuple z} \phi^{\sA}$ of $(m-r)$-tuples in $\sB$, an orbit $O_1 \in C$ and an orbit $O_2 \in D \setminus C$ such that the projection of both $O_1$ and $O_2$ to the last $(m-r)$ coordinates equals to $P$.
The graph $B_{\phi}$ is finite and smooth. Observe that for any arc $(O_1,O_2)$ in $\mathcal{B}_{\phi}$ the projection of $O_1$ and $O_2$ to the last $(m-r)$ coordinates is the same orbit $P$.   
It follows that  $\mathcal{B}_{\phi}$ contains two different components such that the projection of any orbit in the union of these two components to the last $(m-r)$ coordinates equals $P$. 

Now, as in the proof of Proposition~\ref{prop:balanced-finite-hard}, let $M$ be the least common multiple of the length of all cycles in $\mathcal{B}_{\phi}$. Then observe that $\mathcal{B}_{\eta}$ with $\eta := \phi^{\circ M}$ 
contains a loop $(O, O)$ always when $O$ is in a component in $\mathcal{B}_{\phi}$. Since any two elements connected in $\mathcal{B}_{\eta}$ are also connected in $\mathcal{B}_{\phi}$,
every component in $\mathcal{B}_{\phi}$ is a union of components in 
$\mathcal{B}_{\eta}$, and hence also $\mathcal{B}_{\eta}$ 
contains a loop for all elements existing in some component of 
$\mathcal{B}_{\eta}$.


Consider  $\psi := \eta^{|\text{orb}(D)|}$, where $\text{orb}(D)$ is the set of orbits of $m$-tuples in $\sB$ contained in $D$,
and observe that $\mathcal{B}_{\psi}$ and $\mathcal{B}_{\eta}$ have the same components, and every component in the former digraph contains all possible arcs.
Now, $\mathcal{B}_{\theta}$ where 
$\theta(u_1, \ldots, u_r,   v_1, \ldots, v_r, v_{r+1}, \ldots, v_m) \equiv
  \psi(u_1, \ldots, u_r, v_1, \ldots, v_r, v_{r+1}, \ldots, v_m) \wedge \psi(v_1, \ldots, v_r, u_{1}, \ldots, u_r, v_{r+1}, \ldots, v_m)$
is a disjoint union of components in $\mathcal{B}_{\psi}$. It follows that $R_{\theta} =\allowbreak \{ (m(\tuple u),$ $ m(\tuple v)) \mid m \in \theta^{\sA} \}$ seen as a relation over orbits of $m$-tuples in $\sB$  is an equivalence relation on a subset of $\text{orb}(D)$ which contains at least two equivalence classes such that for any $O_1, O_2$ in their union the projection of $O_1$ and $O_2$ to the last $(m-r)$ variables is the same. 


For the first-order reduction, it would be natural to reduce from $\csp(\{ 0,1 \}; R_0, R_1, =)$, where $=$ is the equality on $\{ 0, 1\}$, to $\csp(A; R, O_1, O_2)$ where  $R = \{ m(u_1, \ldots, u_r, v_1, \ldots, v_m) \mid m \in \theta^{\sA} \}$ and $O_1, O_2$ are orbits from two different equivalence classes of $R_{\theta}$. The problem is that $O_1$ and $O_2$ may not be \efpp-definable.
Therefore, in addition to $R$, we will need $R_{O_i,-}$ with $i \in [2]$ which is $R$ where $O_i$ is imposed on $(u_1, \ldots, u_r, v_{r+1}, \ldots, v_m)$ such that whenever $\proj_{i,j} O_1 \subseteq \{ (a,a) \mid a \in A \}$, then we identify the corresponding variables.  All other atoms in the pp-definition of $O_1$ are also \efpp-definable, so we can use them in the definition of $R_{O_i, -}$. Similarly, we also need  $R_{-, O_i}$ with $i \in [2]$ which is like $R_{O_i,-}$ but we impose $O_i$ on $(v_1, \ldots, v_m)$. 
Furthermore we need $R_{O_i, O_j}$ with $i,j \in [1,2]$ which is again like $R$ but this time $O_i$ is imposed on  
$(u_1, \ldots, u_r, v_{r+1}, \ldots, v_m)$ and $O_j$ is imposed on $(v_1, \ldots, v_m)$.

Assume without loss of generality that the definition of $R_{O_i,-}$ is over variables
$(u_1, \ldots, u_{q_i},\allowbreak v_{1}, \ldots,\allowbreak v_m)$, the definition of $R_{-,O_i}$ is over variables
$(u_1, \ldots, u_r, v_{1}, \ldots, v_{q_i}, v_{r+1}, \ldots, v_m)$ with $q_i \leq r$.
In the same fashion, the definition of $R_{O_i,O_j}$ with $i,j \in [2]$ is over variables 
$(u_1, \ldots, u_{q_i},\allowbreak v_{1}, \ldots, v_{q_j},\allowbreak u_{r+1}, \ldots, u_m)$.



We will now provide a $2$-ary interpretation with $m$ parameters $\iota$ of the signature $\tau$ containing $R$, $R_{O_i,-}$, $R_{-,O_i}$ and $R_{O_i,O_j}$ with $i,j \in [2]$ in the signature $\sigma = \{R_=, R_0, R_1 \}$.\


Our intention is to interpret an element of a $\sigma$-structure in a $\tau$-structure as a pair consisting of the element and one of the parameters. Thus, we set $\phi_U(\tuple x, \tuple p) \equiv \bigvee_{i = 1}^{m} (x_2 = p_i$) for $\tuple x =(x_1, x_2)$ and $\tuple p = (p_1, \ldots, p_m)$. Then we define an auxiliary formula parametrized by a natural number $q \leq r$:
$$
\eta_q(\tuple x^1,\ldots, \tuple x^q, \tuple x^{r+1}, \ldots, \tuple x^m, \tup p) \equiv \bigwedge_{i,j \in [q]} (x^i_1 = x^j_1)\wedge \bigwedge_{i = r+1}^{m} (x^i_1 = p_i) \wedge \bigwedge_{i=1}^{q} (x^i_2 =  p_i) \wedge \bigwedge_{i=r+1}^{m} (x^i_2 =  p_i)
$$
\noindent which is satisfied by $((x,p_1), \ldots, (x, p_q), (p_{r+1}, p_{r+1}), \ldots, (p_m, p_m))$ for any $x$. 
We now turn to defining the formulae interpreting the relations over $\tau$.
First we set the formula $\phi_{R}({\tuple x}^1,\ \ldots,{\tuple x}^r,{\tuple y}^1,\ \ldots,{\tuple
y}^m,\allowbreak \tuple p)$ to be equivalent to 
$$\eta_r(\tuple x^1,\ \ldots, \tuple x^r, \tuple y^{r+1}, \ldots, \tuple y^{m}, \tup p) \wedge \eta_r({\tuple y}^1,\ \ldots,{\tuple y}^m, \tuple p) \wedge R_=(x_1^1, y_1^1) \wedge \neg R_0(x_1^1) \wedge \neg R_0(y_1^1) \wedge \neg R_1(x_1^1) \wedge \neg R_1(y_1^1).$$ 

\noindent
The interpretation of $R_{O_i,-}$ with $i \in [2]$ 
is 
$\phi_{R_{O_i},-}({\tuple x}^1, \ldots, {\tuple x}^{q_i},{\tuple y}^1,\ \ldots,{\tuple y}^m, \tuple p)$ equivalent to 
$$\eta_{q_i}(\tuple x^1,\ \ldots, \tuple x^{q_i}, \tuple y^{r+1}, \ldots, \tuple y^{m}, \tup p) \wedge \eta_{r}({\tuple y}^1,\ \ldots,{\tuple y}^m, \tuple p) \wedge R_=(x_1^1, y_1^1) \wedge R_i(x_1^1) \wedge \neg R_0(y_1^1) \wedge \neg R_1(y_1^1).$$

\noindent
The interpretation of $R_{-, O_i}$ with $i \in [2]$ 
is 
$\phi_{R_{-, O_i}}({\tuple x}^1, \ldots, {\tuple x}^{r},{\tuple y}^1, \ldots, {\tuple y}^{q_i}, {\tuple y}^{r+1}, \ldots {\tuple y}^m, \tuple p)$ 
equivalent to 
\begin{center}
    \footnotesize
    $$\eta_{r}(\tuple x^1,\ \ldots, \tuple x^{r}, \tuple y^{r+1}, \ldots, \tuple y^{m}, \tup p) \wedge \eta_{q_i}({\tuple y}^1, \ldots, {\tuple y}^{q_i}, {\tuple y}^{r+1}, \ldots {\tuple y}^m, \tuple p) \wedge R_=(x_1^1, y_1^1) \wedge \neg R_0(x_1^1) \wedge \neg R_1(x_1^1) \wedge  R_i(y_1^1).$$
\end{center}


\noindent
Finally, the interpretation of $R_{O_i, O_j}$ with $i,j \in [2]$ 
is 
$\phi_{R_{O_i, O_j}}({\tuple x}^1, \ldots, {\tuple x}^{q_i},{\tuple y}^1, \ldots, {\tuple y}^{q_j}, {\tuple y}^{r+1}, \ldots {\tuple y}^m, \tuple p)$ 
equivalent to 
$$\eta_{q_i}(\tuple x^1,\ \ldots, \tuple x^{q_i}, \tuple y^{r+1}, \ldots, \tuple y^{m}, \tup p) \wedge \eta_{q_j}({\tuple y}^1, \ldots, {\tuple y}^{q_j}, {\tuple y}^{r+1}, \ldots {\tuple y}^m, \tuple p) \wedge R_=(x_1^1, y_1^1) \wedge R_i(x_1^1) \wedge  R_j(y_1^1).$$ \end{proof}

\noindent
The second proposition addresses the case where a model-complete core is expanded by equality.

\begin{proposition}
\label{prop:equalityLhard}
Let $\sA$ be a first-order expansion of a finitely bounded homogeneous model-complete core $\sB$. Suppose that there is an \efpp-definition of $=_{C}(x,y) \equiv C(x) \wedge C(y) \wedge x=y$  in $\sA$ where $C$ is a unary orbit that contains at least two different elements. Then $\csp(\sA)$ is L-hard under first-order reduction.   
\end{proposition} 
\begin{proof}
Let $O_C$ be a binary injective orbit in $\sB$ such that the projection to either of the coordinates is $C$. We will provide a $1$-ary interpretation with no parameters $\iota$ of the signature $\tau = \{ O_C, = \}$ in the signature $\sigma = \{R_=, R_0, R_1 \}$ where $R_=$ is the equality on $\{ 0, 1\}$. We set $\phi_U(x) \equiv \text{TRUE}$ for the interpretation of the universe and
$\phi_{O_C}(x,y) \equiv R_0(x) \wedge R_1(y)$ and $\phi_{=_C}(x,y) \equiv R_=(x,y)$ for the relations.
\end{proof}


==> chapters/04-infinite/intro.tex <==
\label{sect:infinite}

In this section, we prove Theorem~\ref{thm:main}. We start by redefining the notion of an
implication to capture atomic dependencies over tuples of elements.

\begin{definition}[Implication]
  Let $\sA$ be a relational structure, $k, l \in \mathbb{N}$ and $C \subseteq A^k, D
  \subseteq A^l$  be \efpp-definable in $\sA$ and non-empty.
  Let $\tuple u$ and $\tuple v$ be tuples of pairwise different variables of
  length $k$ and $l$, respectively. We say that an \efpp-formula $\phi$ with
  $(\scope(\tuple{u}) \cup \scope(\tuple{v}) \subseteq \Var(\phi))$ is a \emph{$(C,
  \tuple{u},D,  \tuple{v})$-implication in $\sA$} if all of the following hold:
  \begin{enumerate}
    \item $C\subsetneq\proj_{\tuple u}(\phi^{\sA})$,
    \item $D\subsetneq\proj_{\tuple v}(\phi^{\sA})$,
    \item for all $f\in \phi^{\sA}$, it holds that $f(\tuple u)\in C$ implies $f(\tuple v)\in D$,
    \item for all $\tuple a \in D$, there exists $f\in\phi^{\sA}$ such that $f(\tuple
      u)\in C$ and $f(\tuple v)= \tuple a$.
  \end{enumerate} We sometimes write a $(C, D)$-implication if $\tuple u, \tuple v$ are
  irrelevant or understood from the context.  Moreover, we call an implication
  \emph{balanced} if $(C,\allowbreak\proj_{\tuple u}(\phi^{\sA}))$ equals
  $(D,\allowbreak\proj_{\tuple v}(\phi^{\sA}))$.
  \label{def:inf-implication}
\end{definition}

Implications, as defined above, are often composed as follows.

\begin{definition}[Composition] \label{def:composition}
  Let $\sA$ be a relational structure, let $l_C, l_D, l_E \geq 1$, let $C\subseteq
  A^{l_C}, D \subseteq A^{l_D}, E \subseteq A^{l_E}$ be non-empty, let $\phi_1$ be a
  $(C,\tuple u^1,D,\tuple v^1)$-implication in $\sA$, and let $\phi_2$ be a $(D,\tuple
  u^2,E,\tuple v^2)$-implication in $\sA$ such that $\proj_{\tuple{v^1}} \phi_1^{\sA} = \proj_{\tuple{u^2}} \phi_2^{\sA}$. Let $\phi'_2$ be a copy of $\phi_2$ such
  that $\tuple v^1=\tuple u^2$ and so that $\Var(\phi_1)$ and $\Var(\phi'_2)$ do not share
  any other variables. We define $\phi_1\circ\phi_2$ to be the \efpp-formula
  $(\phi_1\wedge \phi'_2)$. 
  
  Let $\psi$ be a $(C,\tuple u,C,\tuple v)$-implication. 
  For
  $n\geq 2$, we write $\psi^{\circ n}$ for the \efpp-formula $\psi\circ \cdots \circ
  \psi$ where $\psi$ appears exactly $n$ times.
\end{definition}

\noindent
We will now define a few important properties of the implication that are helpful in proofs.

\begin{definition}[Propriety] \label{def:proper}
  We say that a $(C, \tuple{u},D, \tuple{v})$-implication with $\tuple z$ satisfying
  $\scope(\tuple z) = \scope(\tuple u) \cap \scope(\tuple v)$ is \emph{proper} if $\proj_{\tuple z}
  \phi^{\sA} = \proj_{\tuple z} (C(\tuple u))^{\sA} = \proj_{\tuple z} (D(\tuple v))^{\sA}$.
\end{definition}

For a  $(C, \tuple{u},D,  \tuple{v})$-implication $\phi$ in $\sA$ we define $\pi_{\phi}
\subseteq [k] \times [l]$ to be a binary relation with $(i,j) \in \pi$ if
$u_i$ is the same variable as $v_j$. Since both $\tuple u$ and
$\tuple v$ are tuples of pairwise different variables; it cannot happen that $(i, j), (i, j')
\in \pi_{\phi}$ for $j \neq j'$ or $(j, i), (j', i) \in \pi_{\phi}$ for $j \neq j'$. From which we
conclude, that both $\pi_{\phi}$ and $(\pi_{\phi})^{-1}$ are injective partial functions.
Also notice that $\pi_{\phi_{1} \circ \phi_{2}} = \pi_{\phi_{2}} \circ \pi_{\phi_{1}}$.

\begin{definition}[Nontriviality, Stability] \label{def:stable}
  We say that a $(C, \tuple{u},D,  \tuple{v})$-implication is \emph{nontrivial}
  if neither $\pi_{\phi}$ nor $(\pi_{\phi})^{-1}$ is a total function and that it is
  \emph{stable} if it is nontrivial and $\pi_{\phi}$ is an identity on its domain.
\end{definition}

The following two auxiliary lemmata show that the composition of
implications preserves some properties defined above. A version of the first of the
lemmata is Lemma~31 in~\cite{NagyPW-jonsson}.
\begin{lemma}\label{lemma:implcomp} Let $k\geq 1$ and  $\sA$ be a first-order expansion
  of a $k$-homogeneous 
  structure $\sB$. Let $\phi_1,\phi_2$ be implications
  in $\sA$ as in Definition~\ref{def:composition} with $l_C, l_D, l_E \leq k$.

  Then $\phi:= \phi_1 \circ
  \phi_2$ is a $(C,\tuple u^1,E,\tuple v^2)$-implication in $\sA$ with $\proj_{\tuple
  u^1} \phi^{\sA} = \proj_{\tuple u^1} \phi_1^{\sA}$ and $\proj_{\tuple v^2} \phi^{\sA} =
  \proj_{\tuple v^2} \phi_2^{\sA}$. Moreover, for all orbits $O_1 \subseteq \proj_{\tuple
  u^1}(\phi_1^{\sA})$, $O_3\subseteq \proj_{\tuple v^2}(\phi_2^{\sA})$ in $\sB$,
  $\phi^{\sA}$ contains an $O_1 O_3$-mapping if and only if there exists an orbit $O_2$
  in $\sB$ such that $\phi_1^{\sA}$ contains an $O_1 O_2$-mapping and $\phi_2^{\sA}$
  contains an $O_2 O_3$-mapping.

  Furthermore, if both $\phi_1$ and $\phi_2$ are nontrivial
  or proper, then $\phi$ is also nontrivial or proper, respectively, and if both
  $\phi_1, \phi_2$ are both balanced and stable, then also $\phi$ is balanced and stable.
\end{lemma}
\begin{proof} 
  Let $m_1$ be an $O_1 O_2$-mapping in $\phi_1^{\sA}$ and $m_2$ an $O_2 O_3$-mapping
  in $\phi_2^{\sA}$. Since $l_D \leq k$ and $\sA$ is $k$-homogeneous, there is an
  automorphism $\alpha \in \Aut(\sB)$ sending $m_1(\tuple v^1)$ to $m_2(\tuple u^{2})$.
  It follows that $\phi$ contains an $O_1O_3$-mapping $m: \Var(\phi) \to A$ satisfying
  $m(\tuple u^1) = \alpha(m_1(\tuple u^1))$ and $m(\tuple v^2) = m_2(\tuple v^2)$. On the
  other hand, if $m$ is an $O_1 O_3$-mapping in $\phi^{\sA}$, then by the definition of
  $\phi$ we have that $m(\tuple v^1) = m(\tuple u^2)$ in $O_2$ for some orbit $O_2 \in
  \proj_{\tuple v^1} \phi^{\sA}$. Then $\phi_1$ contains an $O_1O_2$-mapping and $\phi_2$
  an $O_2 O_3$-mapping. It is now straightforward to verify that $\phi$ is a $(C, \tuple
  u^1, E, \tuple v^2)$-implication with $\proj_{\tuple u^1} \phi^{\sA} = \proj_{\tuple
  u^1} \phi_1^{\sA}$ and $\proj_{\tuple v^2} \phi^{\sA} = \proj_{\tuple v^2}
  \phi_2^{\sA}$.

  If $\phi_1$ is nontrivial, then $\pi_{\phi_{1}}$ is a partial function and hence $\pi_{\phi_{1} \circ \phi_{2}} =
  \pi_{\phi_{2}} \circ \pi_{\phi_{1}}$ is also a partial function. It follows that $\phi$ is nontrivial provided both $\phi_1$ and $\phi_2$ are nontrivial. 

  Let now $\tuple z^{1}$, $\tuple z^{2}$ and $\tuple z$ be such that $\scope(\tuple z^1) =
  \scope(\tuple u^1) \cap \scope(\tuple v^1)$, $\scope(\tuple z^2) = \scope(\tuple u^2) \cap \scope(\tuple v^2)$
  and $\scope(\tuple z) = \scope(\tuple u^1) \cap \scope(\tuple v^2)$. Notice that $\scope(\tuple z)$ equals to
  $\scope(\tuple z_{1}) \cap \scope(\tuple z_{2})$.
  Let now both \efpp-formulae $\phi_1$ and $\phi_2$ be proper. It follows that
  $\proj_{\tuple z^1} \phi_1^{\sA} = \proj_{\tuple z^1} (C(\tuple u^1))^{\sA} =
  \proj_{\tuple z^1} (D(\tuple v^1))^{\sA}$ and that $\proj_{\tuple z^2} \phi_2^{\sA} =
  \proj_{\tuple z^2} (D(\tuple u^2))^{\sA} = \proj_{\tuple z^2} (E(\tuple v^2))^{\sA}$.
  To see that $\phi$ is proper, observe that $\proj_{\tuple z} (C(\tuple u^1))^{\sA} = \proj_{\tuple z} \phi_1 = \proj_{\tuple z} \phi_2 =\allowbreak \proj_{\tuple z} (E(\tuple v^2))^{\sA}$. 

  Finally, if both
  $\phi_1$ and $\phi_2$ are balanced and stable, then $\phi$ is clearly balanced but also stable
  since $\pi_{\phi} = \pi_{\phi_1} \circ \pi_{\phi_2}$ is also an identity if both
  $\pi_{\phi_1}$ and $\pi_{\phi_2}$ are.
\end{proof}

\noindent
Finally, we show that one can construct a stable, balanced and proper implication from a nontrivial, balanced and proper one. 

\begin{lemma} \label{lem:obtainingstable} Let $k \geq 1$ and $\sA$ be a first-order expansion of a
  finitely bounded $k$-homogeneous structure and $\phi$ be a nontrivial, balanced and proper $(C,
  C)$-implication in $\sA$. Then $\phi$ \efpp-defines a stable, balanced and proper $(C, C)$-implication in $\sA$.
\end{lemma}
\begin{proof} Let $\phi$ be a balanced, proper and nontrivial $(C, C)$-implication in $\sA$ with $C \subseteq
  A^m$ for some $m \leq k$. Observe that $\pi_{\phi \circ \phi} = \pi_{\phi} \circ
  \pi_{\phi}$. 
  Since both $\pi_{\phi}$
  and $(\pi_{\phi})^{-1}$ is a partial injective function, $\pi_{\phi}$ seen as a digraph is a 
  disjoint union of directed cycles and directed paths. 
  Let now $l$ be a
  common multiple of the lengths of all cycles in $\pi_{\phi}$ greater than $m$. It follows that
  $\pi_{\phi^{\circ l}}$ seen as a digraph is an independent set with some vertices having loops, hence $\phi^{\circ l}$ is a stable $(C,C)$-implication. It is balanced and proper by Lemma~\ref{lemma:implcomp}. 
\end{proof}
